Does a Daily Deal Promotion Signal a Distressed Business? An Empirical Investigation of Small Business Survival

In the last four years, daily deals have emerged from nowhere to become a multi-billion dollar industry world-wide. Daily deal sites such as Groupon and Livingsocial offer products and services at deep discounts to consumers via email and social networks. As the industry matures, there are many questions regarding the impact of daily deals on the marketplace. Important questions in this regard concern the reasons why businesses decide to offer daily deals and their longer-term impact on businesses. In the present paper, we investigate whether the unobserved factors that make marketers run daily deals are correlated with the unobserved factors that influence the business, In particular, we employ the framework of seemingly unrelated regression to model the correlation between the errors in predicting whether a business uses a daily deal and the errors in predicting the business' survival. Our analysis consists of the survival of 985 small businesses that offered daily deals between January and July 2011 in the city of Chicago. Our results indicate that there is a statistically significant correlation between the unobserved factors that influence the business' decision to offer a daily deal and the unobserved factors that impact its survival. Furthermore, our results indicate that the correlation coefficient is significant in certain business categories (e.g. restaurants).

==> groupon.tex <==
\section{Groupon}
\label{sec:groupon}
I modeled the probability of offering a Groupon deal as a function of the ``zip" where the business was operating and the price category. 
I modeled the probability of failure  deal as a function of the number of reviews, the  ``zip" where the business was operating and the price category. 

I preformed SURE of group on and failure. The results shown in Table \ref{table:joint risk} show that the correlation between the error in predicting whether a business does a group deal an the error of whether the business closes is positive $\rho = 0.227$ . The results have a p-value of 0.06 which is significant at the 90\% level. I also performed the regression for the ``Bars" category and got $\rho = 0.279$ and a value of $0.1$ indicating that the results are significant at the 90\% confidence level. 


When i combine the two data sets to get a larger set that has both restaurants and Bars and use the category type as an indicator i get {\bf $\rho = 0.204$ and a p value of 0.03, which is significant at the 90\% level}

%\begin{table}[htdp]
%\caption{Bivariate Regression For Rest and Bars }
%\begin{center}
%
%
%\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
%\begin{tabular}{l*{1}{c}}
%\hline\hline
%                    &\multicolumn{1}{c}{(1)}\\
%                    &\multicolumn{1}{c}{isgroupon}\\
%\hline
%isgroupon           &                     \\
%mygrouponziprisk    &       37.21\sym{***}\\
%                    &      (4.77)         \\
%[1em]
%mygrouponpricerisk  &       23.62\sym{***}\\
%                    &      (4.15)         \\
%[1em]
%1b.btype            &           0         \\
%                    &         (.)         \\
%[1em]
%2.btype             &      -0.274\sym{*}  \\
%                    &     (-2.15)         \\
%[1em]
%Constant            &      -2.898\sym{***}\\
%                    &    (-15.03)         \\
%\hline
%isclosed            &                     \\
%myziprisk           &       7.433\sym{***}\\
%                    &      (6.10)         \\
%[1em]
%mypricerisk         &      -12.49\sym{**} \\
%                    &     (-2.92)         \\
%[1em]
%reviewnumber        &    -0.00253\sym{***}\\
%                    &     (-4.67)         \\
%[1em]
%Constant            &       0.229         \\
%                    &      (0.28)         \\
%\hline
%athrho              &                     \\
%Constant            &       0.205\sym{*}  \\
%                    &      (2.13)         \\
%\hline
%Observations        &        2369         \\
%\hline\hline
%\multicolumn{2}{l}{\footnotesize \textit{t} statistics in parentheses}\\
%\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
%\end{tabular}
%
%\end{center}
%\label{table:jointrisk}
%\end{table}%




